I'm Me, We're Us, and I'm Us: Tri-directional Contrastive Learning on Hypergraphs

Although machine learning on hypergraphs has attracted considerable attention, most of the works have focused on (semi-)supervised learning, which may cause heavy labeling costs and poor generalization. Recently, contrastive learning has emerged as a successful unsupervised representation learning method. Despite the prosperous development of contrastive learning in other domains, contrastive learning on hypergraphs remains little explored. In this paper, we propose TriCL (Tri-directional Contrastive Learning), a general framework for contrastive learning on hypergraphs. Its main idea is tri-directional contrast, and specifically, it aims to maximize in two augmented views the agreement (a) between the same node, (b) between the same group of nodes, and (c) between each group and its members. Together with simple but surprisingly effective data augmentation and negative sampling schemes, these three forms of contrast enable TriCL to capture both microscopic and mesoscopic structural information in node embeddings. Our extensive experiments using 13 baseline approaches, five datasets, and two tasks demonstrate the effectiveness of TriCL, and most noticeably, TriCL consistently outperforms not just unsupervised competitors but also (semi-)supervised competitors mostly by significant margins for node classification. The code and datasets are available at https://github.com/wooner49/TriCL.

==> 03_prelim.tex <==
% \section{Preliminaries}
% \label{sec:prelim}
% In this section, we give some preliminaries on hypergraphs and hypergraph neural networks. 


% \paragraph{Hypergraphs and notation.} 
% % A \textit{hypergraph} is a generalized graph that can model higher-order relationships among nodes by allowing an edge, called a hyperedge, to join any number of nodes, unlike conventional graphs where an edge can only model a pair-wise relationship between two nodes. 
% A \textit{hypergraph}, a set of hyperedges, is a natural extension of a graph, allowing the hyperedge to contain any number of nodes.
% Let $H=(V,E)$ be a hypergraph, where $V=\{v_{1},v_{2},\dots,v_{n}\}$ is a set of nodes and $E=\{e_{1},e_{2},\dots,e_{m}\}$ is a set of hyperedges, with each hyperedge is a non-empty subset of $V$.
% The node feature matrix is represented by $\matX\in\bbR^{|V|\times F}$, where $\vecx_{v}\in\bbR^{F}$ is the feature of node $v$.
% In general, a hypergraph can alternatively be represented by its \textit{incidence matrix} $\matH\in\{0,1\}^{|V|\times |E|}$, with entries defined as $h_{ve}=1$ if $v\in e$, and $h_{ve}=0$ otherwise. 
% In other words, $h_{ve}=1$ when node $v$ and hyperedge $e$ form a \textit{membership}.
% % The total number of node-hyperedge memberships is represented by $K=nnz(\matH)$.
% Each hyperedge $e\in E$ is assigned a positive weight $w_{e}$, and all the weights formulate a diagonal matrix $\matW\in\bbR^{|E|\times |E|}$.
% We use the diagonal matrix $\matD_{V}$ to represent the degree of vertices, where its entries $d_{v}=\sum_{e}{w_{e}h_{ve}}$.
% Also we use the diagonal matrix $\matD_{E}$ to denote the degree of hyperedges, where its element $\delta_{e}=\sum_{v}{h_{ve}}$ represents the number of nodes connected by the hyperedge $e$.



% \paragraph{Hypergraph neural networks.}
% Modern hypergraph neural networks~\citep{feng2019hypergraph,yadati2019hypergcn,bai2021hypergraph,dong2020hnhn,arya2020hypersage,chien2021you} follow a two-stage neighborhood aggregation strategy: node-to-hyperedge and hyperedge-to-node aggregation. 
% They iteratively update the representation of a hyperedge by aggregating representations of its incident nodes and the representation of a node by aggregating representations of its incident hyperedges.
% Let $\matP\in\bbR^{|V|\times F'}$ and $\matQ\in\bbR^{|E|\times F''}$ be the node and hyperedge representations, respectively.
% Formally, the $k$-th layer of a hypergraph neural network is 
% \begin{equation}\label{eq:hypergnn}
%     \vecq_{e}^{(k)}=f_{V\rightarrow E}^{(k)}\Big(\vecq_{e}^{(k-1)},\big\{\vecp_{v}^{(k-1)}:v\in e\big\}\Big),\quad
%     \vecp_{v}^{(k)}=f_{E\rightarrow V}^{(k)}\Big(\vecp_{v}^{(k-1)},\big\{\vecq_{e}^{(k)}:v\in e\big\}\Big)
% \end{equation}
% % where $\vecp_{v}^{(k)}$ and $\vecq_{e}^{(k)}$ are node and hyperedge representation at the $k$-th layer, respectively, and $\vecq_{v}^{(0)}=\vecx_{v}.$
% where $\vecq_{v}^{(0)}=\vecx_{v}$.
% The choice of $f_{V\rightarrow E}(\cdot)$ and $f_{E\rightarrow V}(\cdot)$ is critical and a number of models have been proposed.
% In HGNN~\citep{feng2019hypergraph}, for example, they choose $f_{V\rightarrow E}$ and $f_{E\rightarrow V}$ to be the weighted sum over inputs with normalization with node and hyperedge degrees as:
% \begin{equation}\label{eq:hgnn}
%     \vecq_{e}^{(k)}=\sum_{v\in e}{\frac{\vecp_{v}^{(k-1)}}{\sqrt{d_{v}}}},\quad
%     \vecp_{v}^{(k)}=\sigma\bigg(\frac{1}{\sqrt{d_{v}}}\sum_{e:v\in e}\frac{w_{e}\vecq_{e}^{(k)}\mathbf{\Theta}^{(k)}}{\delta_{e}}+\vecb^{(k)}\bigg),
% \end{equation}
% where $\mathbf{\Theta}^{(k)}$ is a learnable weight matrix, $\vecb^{(k)}$ is a bias, and $\sigma$ denote a non-linear activation function.
% Many other hypergraph neural networks can be represented similarly to (\ref{eq:hypergnn}).

























% Aggregation rules can be formally represented by multiset functions~\citep{chien2021you}.
% A multiset function is a \textit{permutation-invariant} function which is the output of the function should not change under arbitrary permutation of the elements in the input set.
% Let $V_{e,\matP}=\{\matP_{u,:}:u\in e\}$ be the multiset of node representations contained in the hyperedge $e$, and $E_{v,\matQ}=\{\matQ_{e,:}:v\in e\}$ be the multiset of hyperedge representations that contain the node $v$. 
% % We use the superscript $(l)$ to indicate that each notation corresponds to the $l$-th layer.
% Then the node-to-hyperedge and hyperedge-to-node message propagation at $l$-th layer use the following update rules, respectively:
% \begin{equation}\label{eq:hypergnn}
% \matQ_{e,:}^{(l+1)}=f_{V\rightarrow E}\big(V_{e,\matP^{(l)}};\matQ_{e,:}^{(l)}\big),\quad 
% \matP_{v,:}^{(l+1)}=f_{E\rightarrow V}\big(E_{v,\matQ^{(l+1)}};\matP_{v,:}^{(l)}\big),
% \end{equation}
% where $f_{V\rightarrow E}$ and $f_{E\rightarrow V}$ are two multiset functions with respect to their first input.
% To sum up, a hypergraph encoder produces a representation of hyperedge $e$ by aggregating representations of incident nodes and hyperedge itself and a representation of node $v$ by aggregating representations of incident hyperedges and node itself.
% In short, hyperedge embedding represents an embedding of a set of nodes and vice versa.






% By (\ref{eq:hypergnn}), it is possible to obtain the representation of hyperedges (i.e. set of nodes) and nodes.
% In this way, it is possible to naturally obtain the representation of hyperedges (i.e. set of nodes).

% For our proposed method, we use a simple hypergraph neural network layer as a special instance of (\ref{eq:hypergnn}).
% We choose $f_{V\rightarrow E}$ and $f_{E\rightarrow V}$ according to
% \begin{equation}\label{eq:encoder}
% \matZ_{e}^{(l+1)}=\sigma\bigg(\sum_{u\in e}{\frac{\matX_{u}^{(l)}}{\delta_{e}}}\mathbf{\Theta}_{E}^{(l)}+\mathbf{b}_{E}^{(l)}\bigg),\quad
% \matX_{v}^{(l+1)}=\sigma\bigg(\sum_{e:v\in e}{\frac{w_{e}\matZ_{e}^{(l+1)}}{d_{v}}}\mathbf{\Theta}_{V}^{(l)}+\mathbf{b}_{V}^{(l)}\bigg),
% \end{equation}
% where $\mathbf{\Theta}_{E}^{(l)}\in\bbR^{F\times F'}$ and $\mathbf{\Theta}_{V}^{(l)}\in\bbR^{F'\times F}$ are learnable weight matrices, $\mathbf{b}_{E}^{(l)}\in\bbR^{F'}$ and $\mathbf{b}_{V}^{(l)}\in\bbR^{F}$ are biases, and $\sigma$ denote a nonlinear activation function.
% (\ref{eq:encoder}) can be represented as (\ref{eq:encoder:matrix}) in matrix form.
% \begin{equation}\label{eq:encoder:matrix}
% \matZ_{E}^{(l+1)}=\sigma\big(\matD_{E}^{-1}\matH^{T}\matX_{V}^{(l)}\mathbf{\Theta}_{E}^{(l)}+\mathbf{b}_{E}^{(l)}\big),\quad
% \matX_{V}^{(l+1)}=\sigma\big(\matD_{V}^{-1}\matH\matW\matZ_{E}^{(l+i)}\mathbf{\Theta}_{V}^{(l)}+\mathbf{b}_{V}^{(l)}\big).
% \end{equation}







% \begin{equation}\label{eq:hypergnn}
% \begin{split}
%     & \vecq_{e}^{(k)}=\textrm{COMBINE}_{V\rightarrow E}^{(k)}\Big(\vecq_{e}^{(k-1)},\textrm{AGGREGATE}_{V\rightarrow E}^{(k)}\big(\{\vecp_{v}^{(k-1)}:v\in e\}\big)\Big), \\
%     & \vecp_{v}^{(k)}=\textrm{COMBINE}_{E\rightarrow V}^{(k)}\Big(\vecp_{v}^{(k-1)},\textrm{AGGREGATE}_{E\rightarrow V}^{(k)}\big(\{\vecq_{e}^{(k)}:v\in e\}\big)\Big),
% \end{split}
% \end{equation}

==> tables/accuracy2.tex <==
\begin{table*}
    % \vspace{-2mm}
    \caption{Node classification accuracy in percentage along with standard deviations. 
    Graph algorithms, marked as $\star$, are applied after converting hypergraphs to graphs via clique expansion.
    For each dataset, the highest and the second-highest performance is highlighted in \textbf{boldface} and \underline{underlined}, respectively.
    A.R. denotes average rank, Time-out represents cases where results are not obtained within 24 hours, and OOM indicates out of memory on a 24GB GPU. 
    % Note that only the listed datasets are used to compute average rank.
    }
    \label{tab:accuracy2}
    \centering
    \scalebox{0.8}{
        \begin{tabular}{clcccccc}
            \toprule
            % \multirow{2}{*}{} & \multirow{2}{*}[-1mm]{Method} & \multicolumn{3}{c}{Co-citation Data} & \multicolumn{2}{c}{Co-authorship Data} & \multirow{2}{*}[-1mm]{A.R.$\downarrow$} \\
            & Method & Zoo & 20News & Mushroom & NTU2012 & ModelNet40 & A.R.$\downarrow$ \\
            % \cmidrule(lr){3-5} \cmidrule(lr){6-7}
            % & & Cora & Citeseer & Pubmed & Cora & DBLP \\
            \midrule
            \midrule
            \multirow{10}{*}{\rotatebox{90}{Supervised}} 
                & \MLP              & 75.62 $\pm$ 9.47  & 79.19 $\pm$ 0.45  & 99.58 $\pm$ 0.29  & 65.17 $\pm$ 2.32  & 93.75 $\pm$ 0.61  & 8.8   \\
                & \GCN\!$^{\star}$  & 36.79 $\pm$ 9.59  & OOM               & 92.47 $\pm$ 0.89  & 71.17 $\pm$ 2.36  & 91.67 $\pm$ 0.21  & 13    \\
                & \GAT\!$^{\star}$  & 36.48 $\pm$ 10.0  & OOM               & OOM               & 70.94 $\pm$ 2.55  & 91.43 $\pm$ 0.26  & 14.7  \\
                & \HGNN             & 78.58 $\pm$ 11.1  & 80.15 $\pm$ 0.25  & 98.59 $\pm$ 0.48  & 72.03 $\pm$ 2.41  & 92.23 $\pm$ 0.16  & 7     \\
                & \HyperConv        & 62.53 $\pm$ 14.5  & 79.83 $\pm$ 0.36  & 97.56 $\pm$ 0.64  & 72.62 $\pm$ 2.64  & 91.84 $\pm$ 0.14  & 9.4   \\
                & \HNHN             & 78.89 $\pm$ 10.2  & 79.51 $\pm$ 0.43  & \textbf{99.78 $\pm$ 0.10}  & 71.45 $\pm$ 3.16  & 92.96 $\pm$ 0.17  & 7     \\
                & \HyperGCN         & 40.86 $\pm$ 2.10  & 77.31 $\pm$ 6.04  & 48.26 $\pm$ 0.26  & 46.05 $\pm$ 3.91  & 69.23 $\pm$ 2.83  & 14.2  \\
                & \HyperSAGE        & 40.86 $\pm$ 2.10  & Time-out          & Time-out          & Time-out          & Time-out          & -     \\
                & \UniGCN           & 72.10 $\pm$ 12.1  & \textbf{80.24 $\pm$ 0.36}  & 98.84 $\pm$ 0.53  & 73.27 $\pm$ 2.69  & 94.62 $\pm$ 0.19  & 6.2   \\
                & \AllSet           & 72.72 $\pm$ 11.8  & 79.90 $\pm$ 0.43  & \underline{99.78 $\pm$ 0.13}  & 75.09 $\pm$ 2.50  & 96.85 $\pm$ 0.21  & 4.8   \\
            \midrule
            \multirow{8}{*}{\rotatebox{90}{Unsupervised}}
                & \Nodetovec\!$^{\star}$  & 17.02 $\pm$ 4.12  & 63.35 $\pm$ 1.74    & 88.16 $\pm$ 0.77  & 67.72 $\pm$ 2.13  & 84.94 $\pm$ 0.44  & 15    \\
                & \DGI\!$^{\star}$        & 36.54 $\pm$ 9.67  & OOM                 & OOM               & 72.01 $\pm$ 2.51  & 92.18 $\pm$ 0.20  & 12.3  \\
                & \GRACE\!$^{\star}$      & 37.07 $\pm$ 9.30  & OOM                 & OOM               & 70.51 $\pm$ 2.38  & 90.68 $\pm$ 0.25  & 14.3  \\
                & \HHGR                 & \underline{80.06 $\pm$ 11.1}  & 79.75 $\pm$ 0.32      & 97.15 $\pm$ 0.49  & 73.95 $\pm$ 2.44  & 93.26 $\pm$ 0.18  & 7.2   \\
                \cmidrule{2-8}
                & \RandomInit           & 78.43 $\pm$ 11.0  & 77.14 $\pm$ 0.58  & 97.40 $\pm$ 0.58  & 74.39 $\pm$ 2.57  & 96.29 $\pm$ 0.28  & 7.8   \\
                & \textbf{\methodN}     & 79.77 $\pm$ 10.9  & 80.14 $\pm$ 0.23  & 99.54 $\pm$ 0.23  & 75.11 $\pm$ 2.52  & 97.01 $\pm$ 0.15  & 4.2   \\
                & \textbf{\methodNE}    & 79.99 $\pm$ 10.9  & 80.17 $\pm$ 0.22  & 99.65 $\pm$ 0.19  & \underline{75.14 $\pm$ 2.51}  & \underline{97.02 $\pm$ 0.14}  & \underline{2.6}   \\
                & \textbf{\method}      & \textbf{80.11 $\pm$ 11.1}  & 80.12 $\pm$ 0.20  & 99.67 $\pm$ 0.19  & \textbf{75.17 $\pm$ 2.49}  & \textbf{97.08 $\pm$ 0.13}  & \textbf{2.2}   \\
            \bottomrule
        \end{tabular}
    }
\end{table*}
